Combinatorial Koszul Homology: Computations and Applications

With a particular focus on explicit computations and applications of the Koszul homology and Betti numbers of monomial ideals, the main goals of this thesis are the following: Analyze the Koszul homology of monomial ideals and apply it to describe the structure of monomial ideals. Describe algorithms to perform efficient computations of the homological invariants of monomial ideals. Apply the theory and computations on monomial ideals to problems inside and outside mathematics The thesis introduces as a main tool Mayer-Vietoris trees of monomial ideals.

==> notations.tex <==

\chapter*{Notations}
\spanishchapter{Notaciones}

The following notations and conventions will be used in the following pages:
\begin{multicols}{2}
\begin{itemize}
\item $\NN$ denotes the set of natural numbers including zero: $\{0,1,2,3,\dots\}$
\item $\kb$ will be a field of characteristic $0$
\item $R=\kb[x_1,\dots,x_n]$ denotes the polynomial ring on $n$ variables over $\kb$
\item $\xb^\mu$ will denote a power product; a power product times a scalar is a monomial
\item $supp(\xb^\mu)$ denotes the support of a monomial or a power product, i.e. the variables wich have non-zero exponent in $\mu$
\item $\preceq$ denotes divisibility among multi-indices
\item $\mm$ denotes the irrelevant ideal of $R$, i.e. $\mm=\langle x_1,\dots,x_n\rangle$ 
\item $\Vc$ denotes an $n$-dimensional $\kb$-vector space
\item $\KK$ denotes the Koszul complex
\item $\KK(\Mc)$ denotes the Koszul complex of the module $\Mc$
\item $\mathfrak{S}\Vc$ denotes the symmetric coalgebra of $\Vc$
\item $I=(m_1,\dots,m_r)=\langle m_1,\dots,m_r\rangle$ is the monomial ideal generated by the monomials $m_1,\dots,m_r$
\item $log(x^\mu)=\mu$ is the map that stablishes the correspondence between the set of all monomials in $R=\kb[x_1,\dots,x_n]$ and $\NN^n$, mapping the exponent of a monomial to its correspondent multiindex
\item $L_I$ denotes the $lcm$ lattice of the monomial ideal $I$; $L_{I,i}$ is the set of elements of $L_I$ given by $lcm$s of exactly $i$ minimal generators of $I$
\item $\PP: \cdots \Pc_i\stackrel{\delta_i}{\rightarrow}\Pc_{i-1}\rightarrow\cdots\rightarrow\Pc_1\stackrel{\delta_i}{\rightarrow}\Pc_{0}\rightarrow 0$ denotes a resolution
\item $\beta_i$ is the $i$-th Betti number and $\beta_{i,\ab}$ denotes the $i$-th Betti number in multidegree $\ab$
\item $\TT$ the Taylor resolution, $\LL$ the Lyubeznik resolution
\item $\langle \cdot, \cdot \rangle$ the scalar product
\end{itemize}

\end{multicols}
